FMViz: Visualizing Tests Generated by AFL at the Byte-level

Software fuzzing is a strong testing technique that has become the de facto approach for automated software testing and software vulnerability detection in the industry. The random nature of fuzzing makes monitoring and understanding the behavior of fuzzers difficult. In this paper, we report the development of Fuzzer Mutation Visualizer (FMViz), a tool that focuses on visualizing byte-level mutations in fuzzers. In particular, FMViz extends American Fuzzy Lop (AFL) to visualize the generated test inputs and highlight changes between consecutively generated seeds as a fuzzing campaign progresses. The overarching goal of our tool is to help developers and students comprehend the inner-workings of the AFL fuzzer better. In this paper, we present the architecture of FMViz, discuss a sample case study of it, and outline the future work. FMViz is open-source and publicly available at https://github.com/AftabHussain/afl-test-viz.

==> future-directions.tex <==
\section{Future Directions}

Potential future directions of this work include:

\begin{comment}
\begin{itemize}
    \item Observe byte-level mutation patterns for different segments of a fuzzing campaign, more multiple input test cases. 
    \item Enhancing this tool by adding color codes for specific \textit{types of mutations}. Currently the tool only visualizes the byte location of a testcase where the mutation was applied, not the type of mutation (e.g. increment, decrement, bitflip, etc.).
    \item Add a feature to allow developers to selectively visualize bytes of interest in a testcase (e.g. the text bytes in an ELF file). 
    \item Visually explore correlations between testcase byte mutation-patterns and testcase coverage and crashes.
    \item Visually compare different mutation scheduling algorithms. 
\end{itemize}
\end{comment}
